Long-range interactions in the avalanches of elastic interfaces

Disordered systems submitted to a slowly increasing external stress often reacts with a jerky dynamics characterized by bursts of activity, called avalanches, which are the manifestation of an out-of-equilibrium phase transition. This thesis focuses on the dynamics of elastic interfaces near the depinning transition, and more specially on the effect of long-range interactions. I derive the universal scaling form of the correlation functions of the local velocity field. It allows to test the universality class of the transition as well as the range of the interactions. I also study the statistics of the clusters that form in presence of long-range interactions and show how it relates to the statistics of the global avalanches. Finally I present analytical advances towards the understanding of the spatial structure of avalanches within a mean-field model, the Brownian force model.

==> notations.tex <==
\glsxtrnewsymbol[description={Positive numbers: $\left[0,+\infty\right[$}]{arr}{$\R_+$}
\glsxtrnewsymbol[description={Expectation with respect to a random variable}]{a}{$\E$}
\glsxtrnewsymbol[description={Average over disorder}]{fda}{$\overline{\cdots}$}
\glsxtrnewsymbol[description={Heaviside Theta function}]{ruzzzt}{$\theta(x)$}
\glsxtrnewsymbol[description={Gamma function}]{ruzzt}{$\Gamma(x)$}
\glsxtrnewsymbol[description={Lambert $W$ function}]{lambw}{$W(x)$}
\glsxtrnewsymbol[description={Airy function}]{laiai}{$\Ai(x)$}
\glsxtrnewsymbol[description={Polylogarithm of order $s$}]{lilisi}{$\Li_s(x)$}
\glsxtrnewsymbol[description={Riemann zeta function}]{lildsisi}{$\zeta(x)$}
\glsxtrnewsymbol[description={Error function: ${\rm Erf}(x)=\frac{2}{\sqrt{\pi}}\int_0^z \rmd t \, e^{-t^2}$}]{laerrmbw}{${\rm Erf}(x)$}
\glsxtrnewsymbol[description={Complementary error function: ${\rm Erfc}(x)=1-{\rm Erf}(x)$}]{laerrfcmbw}{${\rm Erfc}(x)$}
\glsxtrnewsymbol[description={$\max(0,x)$}]{lamaax}{$(x)_+$}
\glsxtrnewsymbol[description={Cauchy principal value}]{lamezaax}{$\dashint$}
\glsxtrnewsymbol[description={Pfaffian}]{pffdf}{${\rm Pf}$}
\glsxtrnewsymbol[description={}]{ruzsdq}{}
\glsxtrnewsymbol[description={Brownian Bridge}]{brobri}{BB}
\glsxtrnewsymbol[description={Brownian Motion}]{bromo}{BM}
\glsxtrnewsymbol[description={Directed Polymer}]{directedPol}{DP}
\glsxtrnewsymbol[description={Gaussian Beta Ensemble of Random Matrix Theory}]{GGbE}{G$\beta$E}
\glsxtrnewsymbol[description={Gaussian Orthogonal Ensemble}]{GGOE}{GOE}
\glsxtrnewsymbol[description={Gaussian Unitary Ensemble}]{GGUE}{GUE}
\glsxtrnewsymbol[description={Gaussian Symplectic Ensemble}]{GGSE}{GSE}
\glsxtrnewsymbol[description={Joint Probability Distribution Function}]{GGbEdds}{JPDF}
\glsxtrnewsymbol[description={Kardar-Parisi-Zhang}]{ruzzft}{KPZ}
\glsxtrnewsymbol[description={Moment Generating Function}]{ruszq}{MGF}
\glsxtrnewsymbol[description={Probability Distribution Function}]{ruzq}{PDF}
\glsxtrnewsymbol[description={Random Matrix Theory}]{rumtzq}{RMT}
\glsxtrnewsymbol[description={Stochastic Airy Operator}]{rusasa}{SAO}
\glsxtrnewsymbol[description={Stochastic Heat Equation}]{rumshe}{SHE}
\glsxtrnewsymbol[description={Tracy-Widom}]{rutw}{TW}
\glsxtrnewsymbol[description={Wentzel-Kramers-Brilloin}]{rutwkb}{WKB}
\glsxtrnewsymbol[description={Weak Noise Theory}]{rutwnt}{WNT}
